Rebooting Ultrasonic Positioning Systems for Ultrasound-incapable Smart Devices

An ultrasonic Positioning System (UPS) has outperformed RF-based systems in terms of its accuracy for years. However, few of the developed solutions have been deployed in practice to satisfy the localization demand of today's smart devices, which lack ultrasonic sensors and were considered as being `deaf' to ultrasound. A recent finding demonstrates that ultrasound may be audible to the smart devices under certain conditions due to their microphone's nonlinearity. Inspired by this insight, this work revisits the ultrasonic positioning technique and builds a practical UPS, called UPS+ for ultrasound-incapable smart devices. The core concept is to deploy two types of indoor beacon devices, which will advertise ultrasonic beacons at two different ultrasonic frequencies respectively. Their superimposed beacons are shifted to a low-frequency by virtue of the nonlinearity effect at the receiver's microphone. This underlying property functions as an implicit ultrasonic downconverter without throwing harm to the hearing system of humans. We demonstrate UPS+, a fully functional UPS prototype, with centimeter-level localization accuracy using custom-made beacon hardware and well-designed algorithms.

==> sections/motivation.tex <==


\section{Related Work}
\label{section:motivation}

We review the related work from two aspects: the designs of hash functions and hash enabled protocols.

\textbf{Design of hash function.} Feldhofer and Rechberger \cite{feldhofer2006case} firstly point that current common hash functions (\eg \texttt{MD5}, \texttt{SHA-1}, \etc), are not hardware friendly and unsuitable at all for RFID tags, which have very constrained computing ability.   Such difficulty has spurred considerable research \cite{feldhofer2006case,yoshida2007mame,bogdanov2007present,rolfes2008ultra,bogdanov2007present,poschmann2007new,lim2005mcrypton,yusecurity,hong2006hight,poschmann2007new,good2007hardware}. We sketch the primary designs and their features in Table.~\ref{tab:hash-comparision}. For example, Bogdanov \etal \cite{bogdanov2007present} propose a hardware-optimized block cipher, PRESENT, designed with area and power constraints.  The follow-up work \cite{rolfes2008ultra} presents three different architectures of PRESENT and highlights their availability for both active and passive smart devices. Their implementations reduce the number of GEs to $1,000$ around. 
%Another follow-up work \cite{bogdanov2008hash} extends the design of PRESENT and gives 8 variants to fulfill different requirements, \eg DM-PRESENT-80, DM-PRESENT-128, H-PRESENT-128, \etc\  The work \cite{poschmann2007new} suggests to choose DES as hash function for RFID tags due to relatively low complexity, and presents a variant of DES, called as\ie DESXL. 
Lim and Korkishko \cite{lim2005mcrypton} present a $64$-bit hash function with three key size options ($64$ bits, $96$ bits and $128$ bits),  which requires  about $3,500$ and $4,100$ GEs.  In summary, despite these optimized designs, majority are still presented in theory and  none of them are available for the COTS RFID tags. On contrary, our work explores hash function from another different aspect, that is, leveraging selective reading to mimic equivalent hash primitives.

\begin{table}[!t]
  \centering
  \caption{Performance overview of current hash functions  \protect \footnotemark}
  \label{tab:hash-comparision}
  \vspace{-0.3cm}
  \footnotesize
  \begin{tabular}{|l|c|c|c|c|}
    \hline
    \textbf{Hash functions} & \textbf{Key size}&\textbf{GE} & \textbf{Power} & \textbf{Clock cycles} \\
    \hline
     SHA-256\cite{feldhofer2006case} &256& 10,868 &15.87$\mu A$  & 1,128 \\
     \hline
     SHA-1 \cite{feldhofer2006case}& 160&8,120 & 10.68$\mu A$  & 1,274\\
     \hline
     AES \cite{feldhofer2004strong} &128&  3,400 &8.15$\mu A$  & 1,032 \\
     \hline
     MAME\cite{yoshida2007mame} & 256&8,100 &5.16$\mu A$  & 96 \\
     \hline
     MD5 \cite{feldhofer2006case}& 128& 8,400 & -  & 612 \\
     \hline
     MD4 \cite{feldhofer2006case} & 128& 7,350 & -  & 456 \\
     \hline
     PRESENT-80 \cite{bogdanov2007present} & 80& 1,570 & -  & 32 \\
     \hline
     PRESENT-80 \cite{rolfes2008ultra} & 80&1,075 & -  & 563 \\
     \hline
     PRESENT-128 \cite{bogdanov2008hash} & 128&1,886 & -  & 32 \\     
     \hline
     DES \cite{poschmann2007new} & 56 &2,309 & -  & 144 \\
     \hline
     mCrypton \cite{lim2005mcrypton} & 96&2,608 & -  & 13 \\
     \hline
     TEA \cite{yusecurity} & 128 &2,355 & -  & 64 \\
     \hline
     HIGHT \cite{hong2006hight} & 128 &3,048 & -  & 34 \\
     \hline
     DESXL \cite{poschmann2007new} & 184 &2,168 & -  & 144 \\
      \hline
     Grain \& Trivium\cite{good2007hardware} & 80 & 2,599 & -  & 1 \\
    \hline
  \end{tabular}
\end{table}

%\footnotetext{ `-' means the algorithm is presented in theory and does not have  specific power consumption.}



\textbf{Design of hash enabled protocol.} To drive our key point, we conduct a brief survey of previous related works. We list several key usage scenarios that we would like to support. Our objective is not to complete the list, but to motivate our design.
(1) \emph{Cardinality estimation.} Dozens of estimators \cite{kodialam2007anonymous,sheng2008finding,sze2009fast,qian2010asap,qian2011cardinality,shah2011cardinality,shahzad2012every,zheng2013zoe,chen2013understanding,xiao2013differential,gong2014arbitrarily,liu2014fast,zheng2014towards,liu2015rfid,hou2015place} have been proposed in the past decade. For example, Qian \etal \cite{qian2011cardinality} proposed an estimation scheme called lottery frame. Shahzad and Liu \cite{shahzad2012every} estimated the number based on the average run-length of ones in a bit string received using the FSA. In particular, they claimed that their protocol is compatible with Gen2 systems. However, their scheme still requires modifying the communication protocol, and thus, it fails to work with COTS Gen2 systems. By contrast, our prototype can operate in COTS Gen2 systems as demonstrated in this study. (2) \emph{Missing detection.} The missing detection problem  was firstly mentioned in \cite{tan2008monitor}. Thereafter,  many follow-up works \cite{li2010identifying,luo2011efficient,zhang2011fast,luo2012probabilistic,zheng2015p,tan2010efficient,li2013efficient,liu2014multiple,luo2014missing,ma2012efficient,xie2014rfid,shahzad2015expecting,shahzad2016fast,yu2016missing,yu2015finding} have started to study the issue of false positives resulting from the collided slots  by using multiple bitmaps. 
(3) \emph{Continuous reading.} The traditional inventory approach starts from the beginning each time it interrogates all the tags, thereby making it highly time-inefficient. These works \cite{sheng2010efficient,xie2013continuous,liu2014towards} have proposed continuous reading protocols that can incrementally collect tags in each step using the bitmap. For example, Sheng \etal \cite{sheng2010efficient} aimed to preserve the tags collected in the previous round and collect only unknown tags. Xie \etal \cite{xie2013continuous} conducted an experimental study on mobile reader scanning. Liu \etal \cite{liu2014towards} initially estimated the number of overlapping tags in two adjacent inventories and then performed an effective incremental inventory.
(4) \emph{Data mining.} These works \cite{sheng2008finding,xie2014efficiently,luo2013efficient,luo2016efficient,liu2015fast} discuss how to discover potential information online through bitmaps. For example,  Sheng \etal  \cite{sheng2008finding} proposed to identify the popular RFID categories using the group testing technique.  Xie \etal found histograms over tags through a small number of bitmaps\cite{xie2014efficiently}. Luo \etal \cite{luo2013efficient,luo2016efficient} determined whether the number of objects in each group was above or below a threshold. Liu \etal \cite{liu2015fast} proposed a new online classification protocol for a large number of groups.
(5) \emph{Tag searching.} These works\cite{liu2015step,zheng2013fast} have studied the tag searching problem that aims to find wanted tags from a large number of tags using bitmaps in a  multiple-reader environment. Zheng \etal  \cite{zheng2013fast} utilized bitmaps to aggregate a large volume of RFID tag information and to search the tags quickly.  Liu \etal \cite{liu2015step}  first used the testing slot technique to obtain the local search result by iteratively eliminating wanted tags that were absent from the interrogation region.
(6) \emph{Tag polling.} \cite{qiao2011energy,qiao2013tag,li2016locp} consider how to quickly obtain the sensing information from sensor-augmented tags. The system requires to assign a time slot to each tag using the presence bitmap. In summary, all the aforementioned HEP designs have allowed RFID research to develop considerably in the past decade.  All the work can be boosted by our hash primitives.



















